VEIL: Vetting Extracted Image Labels from In-the-Wild Captions for Weakly-Supervised Object Detection

The use of large-scale vision-language datasets is limited for object detection due to the negative impact of label noise on localization. Prior methods have shown how such large-scale datasets can be used for pretraining, which can provide initial signal for localization, but is insufficient without clean bounding-box data for at least some categories. We propose a technique to "vet" labels extracted from noisy captions, and use them for weakly-supervised object detection (WSOD), without any bounding boxes. We analyze and annotate the types of label noise in captions in our Caption Label Noise dataset, and train a classifier that predicts if an extracted label is actually present in the image or not. Our classifier generalizes across dataset boundaries and across categories. We compare the classifier to nine baselines on five datasets, and demonstrate that it can improve WSOD without label vetting by 30% (31.2 to 40.5 mAP when evaluated on PASCAL VOC). See dataset at: https://github.com/arushirai1/CLaNDataset.

==> iccv2023AuthorKit/figures/cross_category.tex <==
\begin{figure}
    \centering
    \includegraphics[scale=0.3]{iccv2023AuthorKit/figures/images/cross_cat_black.png}
    %scale=0.62
    \caption{Cross Category Generalization Ability of VEIL when used for vetting for WSOD. We measure Object Detection AP on VOC, and the black solid line represents the median  and the black dotted line represents the mean. It appears that predicted VPEL precision (see Table \ref{tab:cross_category}) plays a strong role in WSOD performance when accounting for outliers.}
    \label{fig:cross_cat}
\end{figure}

==> iccv2023AuthorKit/figures/fig1.tex <==
\begin{figure}
    \centering
    \includegraphics[scale=0.32]{iccv2023AuthorKit/figures/images/figure_1_alt2.png}
    % \caption{Due to the diverse ways in which language is used, literal visual alignment cannot always be guaranteed. Labels  extracted from in-the-wild captions can be visually absent due to structurally and semantically unaware label extraction. Above, we showcase examples from RedCaps and SBUCaps.}
    \caption{A naive label extraction process, e.g. substring matching between class names and caption, can lead to visually absent labels. }
    \label{fig:vael_examples}
\end{figure}

==> iccv2023AuthorKit/figures/label_taxonomy.tex <==
\begin{figure}[t] %[h]   
    \includegraphics[width=1\linewidth]{iccv2023AuthorKit/figures/images/label_tax_font_larger2.png}
    %\includegraphics[scale=0.70] {iccv2023AuthorKit/figures/images/label_noise_taxonomy3.png}
    \caption{Label noise taxonomy outlining common reasons for visual absence in extracted labels from in-the-wild captions.}
    \label{fig:label_noise_taxonomy}
\end{figure}

==> iccv2023AuthorKit/figures/scale.tex <==
\begin{figure}[t] %[h]
    \centering
\includegraphics[width=0.3\textwidth]{iccv2023AuthorKit/figures/images/scale_wsod.png}
    %scale=0.8
    \caption{Pascal VOC-07 detection performance of WSOD models trained on RedCaps.}% with (using VEIL-SBUCaps,CC) and without vetting. }
    \label{fig:scale}
\end{figure}

==> iccv2023AuthorKit/figures/structured_noise_qual.tex <==
\begin{figure}[t] %[h]
    \centering
\includegraphics[width=0.5\textwidth]{}
    %scale=0.8
    \caption{Part and contextual bias found in detections from LLM \cite{Kim2022LargeLM} WSOD model
    (red boxes) compared to full object localized with high confidence by WSOD model trained on data vetted by VEIL-SBUCaps (blue boxes). The categories shown are (clockwise from top-left): car, car, cat, car, boat, bus, bus, car.}
    % adaptive, caption independent approach, LLM \cite{Kim2022LargeLM}.}
    \label{fig:structured_qual}
\end{figure}

==> iccv2023AuthorKit/figures/train_subset_figures.tex <==
% \begin{figure}
%     \centering   
%     %\includegraphics[scale=0.5]{iccv2023AuthorKit/figures/images/prec_train_subset.png}  
%     \includegraphics[scale=0.3]{iccv2023AuthorKit/figures/images/f1_train_subset.png}
%     \includegraphics[scale=0.3]{iccv2023AuthorKit/figures/images/cross_cat_black.png}
%     \caption{This figure shows the impact of pseudo-labeled data size for VEIL-SBUCaps on its performance on SBUCaps-Test VPEL Detection. VEIL only needs 10\% of the data to beat No Vetting,
%     %(XX vs 0.633 F1), 
%     and 50\% of the labeled data (80K samples) to beat CLIP.} %This indicates that we only need a small amount of pseodo-labeled data to beat CLIP in terms of precision and slightly more to improve recall and therefore F1.}
%     \label{fig:train_subset}
% \end{figure}

\begin{figure}
  \centering
  %\subfigure[This figure shows the impact of pseudo-labeled data size for VEIL-SBUCaps on its performance on SBUCaps-Test VPEL Detection. VEIL only needs 10\% of the data to beat No Vetting,
    %(XX vs 0.633 F1),     and 50\% of the labeled data (80K samples) to beat CLIP.]{
    \includegraphics[width=0.2\textwidth]{iccv2023AuthorKit/figures/images/limited_train_data_bigger_2.png}
    %} \subfigure[Caption for subfigure 2]{
    \includegraphics[width=0.2\textwidth]{}
    %}
  \caption{(Left) The impact of pseudo-labeled data size for VEIL-SBUCaps on its performance on SBUCaps-Test vetting. 
  %VEIL only needs 10\% of the data to beat No Vetting, and 50\% of the labeled data (80K samples) to beat CLIP.}
  (Right) Cross-category generalization, comparing of WSOD performance on VOC-07 mAP (over 7 overlapping ID categories) when vetting train data, SBUCaps-Test ID, using VEIL-ID and VEIL-OOD. Dashed line indicates mean AP and solid line is median AP.}
\label{fig:train_subset}
\end{figure}

==> iccv2023AuthorKit/old_files/experiments.tex <==
\section{Experiments}
We evaluate ELaVet under the visual presence binary classification task. To evaluate label quality in this task across multiple vision-language datasets without ground truth image-level labels we compute pseudo-image labels for each image from an ensemble of VINVL and YoloV5 pretrained object detectors. We also test ELaVet as a label noise filtering method for weakly supervised object detection. We mainly benchmark the resulting object detector on PASCAL VOC 2007.

\textbf{ELaVet Training.} For each dataset mentioned in section \ref{}, we filter out any caption without a COCO \cite{} object mention, and then save  80-20 train-test splits. For each train split, we train a separate ELaVet model to predict visual presence/absence for each object mention. Since we don't have ground truth object category available for images from SBUCaps \cite{Ordonez2011Im2TextDI}, RedCaps \cite{Desai2021RedCapsWI}, Conceptual Captions \cite{Sharma2018ConceptualCA}, and VIST \cite{huang2016visual}, we use pseudo-labels from an ensemble of pretrained object detectors. We use YOLOv5 and VinVL's object detection model as we observed higher precision on visual presence classification. We evaluated this on a small 250 subset of hand-annotated visual presence/absence of certain objects (elephant, truck, cake, bus, cow) for each of the following datasets: SBUCaps, RedCaps, and Conceptual Captions. We found that an ensemble between YOLOv5 and VinVL had better performance across these three datasets, so we used these object detectors as ground truth for visual presence (if an object mention is also predicted to be in the image by the object detector).
 
\textbf{Weakly Supervised Object Detection (WSOD) and Evaluation.} We use the test split of SBUCaps as the train data for weakly supervised object detection, because the in-domain ELaVET is trained on the train split of SBUCaps. All noise filtering approaches are integrated as a preprocessing filtering step and the noise correction approaches are integrated to training. We benchmark on Pascal VOC 2007 \cite{everingham_2010} and COCO \cite{Lin2014MicrosoftCC} and use the mAP metric to evaluate both classification and localization ability of the WSOD models. 

We simulate a batch size of 8 for all experiments unless specified otherwise. We trained under different GPU settings (4 TK GPUs, with a batch size of 8 or 4 TK GPUs with a batch size of 4 and gradient accumulation which means that we updated parameters every two iterations simulating a batch size of 8) due to resource availability, and used gradient accumulation for some experiments . %We find that gradient accumulation makes virtually no difference to model performance.

%\subsection{Descriptiveness Score Predictor}



\subsection{Direct evaluation of cleanliness}
\input{iccv2023AuthorKit/tables/direct_eval_by_dataset.tex}
We have the following baselines:\\
\textbf{No filtering.} We apply no filtering technique to the image-caption pairs.\\
\textbf{CLIP-based methods.} We use the ViT-B/32 pretrained CLIP \cite{Radford2021LearningTV} image and text model for these methods. We prepend the entire caption with the following prompt, "A photo depicts" as recommended by CLIPScore \cite{Hessel2021CLIPScoreAR} and then compute the cosine similarity between the image and text embeddings outputted by CLIP. On the train datasets, we train a Gaussian Mixture model with two components. The cluster containing higher scoring image-text pairs is assumed to correspond to higher visual-text alignment. This method is what we call GlobalCLIP, and image-text pairs that are predicted to be more visually aligned are selected. For LocalCLIP, we follow a similar process except instead of computing the cosine similarity between an image and caption, we take the cosine similarity between an image and the prompt ``this is a photo of a" followed by the extracted label. LocalCLIP filters extracted labels whereas GlobalCLIP filters based on the caption, even if there are extracted labels that are visually present. For the ensemble variant, we use a variety of prompts, and prepend each to the caption or extracted label. Then for each image and text (the prompt and caption/extracted label), we calculate the cosine similarity between the image-text CLIP embeddings and use the highest scoring caption.
\\\textbf{Descriptiveness and Narrativeness.} If the text has a descriptiveness score higher than 0.5, the descriptiveness based method selects the caption. However, the narrativeness method does the opposite.
\\\textbf{Rule Based Methods.} These rule based methods are motivated by the fact that a category could be mentioned in a noun phrase (``\textbf{car} park"). The first noun modifier based filters an extracted label if the part-of-speech label is an adjective or is followed directly after by a noun. The second noun modifier rule uses the first rule and also filters if the extracted label is not associated with a noun POS tag.
\\\textbf{LLM Simulation.} LLM \cite{Kim2022LargeLM} is language-agnostic dynamic noisy label selection and correction method. For the purposes of measuring its ability to detect VPELs, we simulate five epochs of WSOD training \cite{bilen2016weakly} and assume any label exceeding the large loss threshold specified in \cite{Kim2022LargeLM} as ``predicted to be visually absent" after the first epoch. 

For most methods there is a significant improvement in precision (except for COCO which is a fairly clean dataset), except selecting based on Descriptiveness or Narrativeness (only one can do better). The performance of the in-domain alignment model is much stronger in terms of precision and recall than the other noise filtering methods on most of the datasets. Additionally, AM Cross-Dataset has better F1 scores compared to CLIP despite not using additional information - image and trained on less than 0.5\% of the data. 

In terms of text only approaches (excluding LLM and CLIP-based methods), both alignment models do better than no filtering and the descriptiveness-based and rule based methods in terms of precision and recall. Cap2Det still achieves better results than no filtering despite being trained on COCO Captions which follow a different input distribution (mainly descriptive) and noise distribution (not as noisy). However, the precision not as strong as AM Cross-Dataset. 

Language conditioned VPEL selection approaches do a better job at improving the quality of samples than an large loss matters. However, LLM has fairly strong recall and at times better precision than non-AM language condiitoned methods. LLM seems to have the least improvement in precision on SBUCaps. Local CLIP-E does better than LLM in terms of precision.

The significant drop in recall between the first noun modifier rule and the second (filtering based on whether the object is a noun) shows that there are enough instances where an object mention might be labeled as not a noun but is still present in the image. This might be due to mislabeling in the POS tag prediction due to domain shifts in these captions. However, on more descriptive texts such as CC, COCO, and VIST-DII there's still a drop in recall, so perhaps its not just due to domain shifts. 

\subsubsection{Knowledge Sharing capability of the Alignment Model}
\textbf{What is the cross-dataset generalization ability of the alignment model?}
From the table there are improvements in terms of precision in 4/5 datasets, and improvements in terms of F1 score in 3/5 compared to no filtering. There may be a few reasons why the model might not generalize to a different dataset, for example difference in data distribution, sentence structure, noise types (prevalence of noun-phrase type errors in dataset - more linguistic structure context needed over non-literal errors - more semantic context needed), or different category distributions. 
\input{iccv2023AuthorKit/tables/cross_dataset_CLIP.tex}
We first investigate applying different levels of masking and predicting based on special token rather than the output embedding associated with the object mention directly to learn more general noise patterns applicable to different objects. We also include CLIP and try to reach the cross-domain performance of CLIP. In Table \ref{}, the AM performance slightly improves when applying special tokens however not as much as CLIP. Interestingly, ensembling CLIP and AM Cross-Dataset produces better precision and recall. This is because TK. CLIP seems to do poorly in cases where ``", however the alignment model predicts a lower score ``". My hypothesis is related to object sense.

\textbf{What is the cross-label generalization ability of the alignment model?}
\input{iccv2023AuthorKit/tables/cross_category.tex}
\begin{figure}
    \centering
    \includegraphics[scale=0.40]{iccv2023AuthorKit/figures/images/cross_category_results.png}
    \caption{The star in red represents the mean.}
    \label{fig:cross_cat}
\end{figure}
We can see that in Table 7, while the precision improves over unfiltered, the recall is fairly low. The special token variant of our approach improves recall significantly, however a gap remains between unfiltered and ID in terms of F1. It appears that the OOD can identify when a label is noisy, however is too strict and object dependent, at least when trained on only 20 object classes.

\subsection{Effect on WSOD}

\textbf{How do all the language conditioned filtering compare against one another?}


\textbf{How do all the filtering approaches compare against adaptive noise correction approaches?}


\input{iccv2023AuthorKit/tables/indirect_evaluation.tex}

% First we establish a baseline by looking at performance when \textbf{No Vetting} is applied. Language-conditioned approaches take the caption as input, and produce a score that is used for selection: descriptiveness score, narrativeness score, rule based variants, Cap2Det, and VEIL. Table \ref{tab:table2_label} shows that precision improves across most of these methods. The exceptions being descriptiveness score predictor (and its complement, narrativeness) which seem very weakly or unrelated to the visual presence of labels, however, descriptiveness improves precision in all the descriptive leaning  datasets (CC, COCO, VIST, VIST-DII). This can be explained by recall significantly dropping on predominantly narrative style datasets (SBUCaps, RedCaps), which means that even though captions may be in a narrative-like style it doesn't mean that we should reject its contents. Similarly, even though the rule-based methods significantly improve precision, they suffer in recall due to sometimes the object mention in the noun phrase might be implied to be present (show example: TK). Seeing the drop in recall and F1, it appears that the second rule is too strict, as there may be situations where an object mention might not be tagged as a noun due to odd sentence structure or ?? (TK find examples). Still, given that the precision is still low, a significant number of visually absent extracted labels fall under other categories that are not easily captured by rules (non-literal, narrative artifact). Cap2Det despite being trained on COCO, still transfers and slightly boosts the precision of labels in out-of-domain settings like SBUCaps, RedCaps, and Conceptual Captions. Unsurprisingly, VEIL Same Dataset beats all methods in the web-sourced datasets when it comes to precision and F1, indicating that despite differences in recall, overall there's a much cleaner pool of labels without rejecting too many. Furthermore, a perfect fit between the ground truth and VEIL's predictions would be undesirable as it would be no better than using an object detector predictions as vetting. It's better to learn general properties of noisy labels because even if they may appear in the data, maybe the example would be difficult as it might not be the main focus. We can see that VEIL Cross Dataset is stronger than any of the language-conditioned approaches in terms of precision and F1, indicating potential for generalization. We will explore this more concretely in the next section.


==> iccv2023AuthorKit/old_files/in_the_wild_captions_vs_descriptive_captions.tex <==
\section{Analysis: Descriptive vs In-the-wild captions}
\label{sec:analysis}

We analyze what makes three large-scale in-the-wild datasets a challenging source of labels for object detection methods.
We use the VIST dataset to demonstrate linguistic differences of narrative and descriptive captions, then show the ratio of narrative captions, and a taxonomy of sources of extracted label noise, in the other four datasets. 
% also describe preprocessing

\textbf{COCO} \cite{Lin2014MicrosoftCC} contains cleanly crowdsourced captions, and stands in for the status quo in weakly supervised object detection since the cost of collecting COCO does not scale well.
Visual Storytelling (\textbf{VIST}) \cite{huang2016visual} contains three styles of captions, of which we use two: \textbf{D}escriptions of \textbf{I}mages in \textbf{I}solation (DII), which are similar to captions commonly used for pretraining for object detection \cite{Lin2014MicrosoftCC,Young2014Flicker30K}, and 
\textbf{S}tory for \textbf{I}mages in \textbf{S}equence (SIS), similar to in-the-wild captions. 
Each image contains both DII and SIS captions, which allows us to observe the impact of caption style while keeping the image constant.
Conceptual Captions (\textbf{CC}) \cite{Sharma2018ConceptualCA}, and the remaining two datasets, are collected from in-the-wild data sources. CC contains 3 million image-alt-text pairs after heavy post-processing; samples were accepted if there was an overlap between Google Cloud Vision API class predictions and the caption and named entities were hypernymized.
\textbf{RedCaps} \cite{Desai2021RedCapsWI} is the largest dataset used in our paper, consisting of 12M image-text pairs collected from Reddit by crawling a manually curated list of subreddits with heavy visual content.
SBU Captioned Photo Dataset (\textbf{SBUCaps}) \cite{Ordonez2011Im2TextDI} consists of 1 million Flickr photos with associated text descriptions written by their owners.
%on the photo-sharing platform. 
%To construct this dataset, 
Only captions with at least one prepositional phrase and at least 2 matches with a predefined vocabulary were accepted.

% Prior work \cite{Alikhani2019CaptionAA} demonstrates linguistic differences between captions produced from crowdsourcing (VIST, COCO, Flickr) and online in-the-wild captions (CC, Recipe).
% %and other written text corpora (ANC, FS). This paper
% It notes that natural captions from VIST-SIS and CC contain ``play-by-play descriptions [...]
% %in the narrative present (or sometimes for VIST, past) 
% rather than the progressive descriptions provided by crowd-workers who just
% describe what they see.'' We hypothesize that this narrative element found in in-the-wild corpora, can impact the visibility of objects mentioned in the caption, and this noise can diminish the ability to successfully train an object detection model. Positive signals are sparse and false positive noise can have a greater impact than false negative noise  \ref{}. This motivates us to more effectively use this widely available form of weak supervision from in-the-wild captions, using VEIL.

\subsection{Descriptive/Narrative Linguistic Differences}
\label{sec:ling_diffs}

%The linguistic structure of a caption may correlate with visual-textual alignment. For example, a caption with a low count of nouns might not mention the salient objects. Prepositions such as ``next to'' may convey spatial information that is likely to be visible. Other prepositions such as ``like'' may indicate the use of non-literal language (figure of speech) and any object that follows will likely \emph{not} to be visible. Discourse relations and tagging content as nucleus (core) or satellite (helper) could inform us that non-visual context is provided, e.g. ``We used the gondolas one night [nucleus; gondolas visible] to go to a ball [satellite; ball not visible]." 

\begin{table}[t] %[!htb]
      \centering
        \small
        \begin{tabular}{r c c}\hline
            Part of Speech \vline & Descriptive (DII) & Narrative (SIS) \\ \hline
            noun \vline & \textbf{3.85} & 2.73 \\
            preposition \vline& \textbf{1.75} & 1.01 \\
            adjective \vline & \textbf{0.98} & 0.85 \\
            personal pronoun \vline & 0.18 & \textbf{0.80} \\%\hline
            %\textbf{verb} \vline &1.55 & \textbf{2.00}\\\hline
            verb base \vline & 0.07 & \textbf{0.37}\\
            verb gerund \vline& \textbf{0.61} & 0.23\\
            past tense \vline& 0.08 & \textbf{0.89}\\
            %past participle \vline&  \textbf{0.21} & 0.17\\
            %non-3rd person sing pres \vline&\textbf{ 0.22}& 0.16\\
            %3rd person sing pres \vline& \textbf{0.36}& 0.19\\
        \end{tabular}
    \caption{Part of speech differences in descriptive/narrative caps. }
    \label{tab:pos_dii_sis}
\end{table}

\noindent\textbf{Part of Speech (POS).}
We extract POS tags over all VIST captions using SpaCy \cite{spacy2} and observe differences in pronoun usage and verb tense between descriptive and narrative captions (Table \ref{tab:pos_dii_sis}). The increased use of pronouns in SIS suggests a deviation from an impersonal, objective tone. For the same image, one SIS caption says ``\textbf{we} finally arrive at the island" while a DII caption provides count and detailed information: ``\textbf{a group of four men} sitting together".
In the supplementary materials, we show verb tense and aspect also differ between descriptive/narrative captions. Present tense is much more common in descriptive captions (81\% in DII vs 47\% in SIS) while past tense is more common in narrative captions (19\% in DII and 53\% in SIS). 
%Further, aspect distribution is also distinct across DII and SIS. Progressive aspect refers to verbs that describe an ongoing activity such as ``The event is starting, there are even some dancers forming outside" (SIS) while perfective describes a completed activity, e.g. ``The old part has been \textbf{removed} and now there many loose wires now" (SIS). 
DII contains mostly progressive captions (95\%) meaning that it describes ongoing activities more likely to be present in the accompanying visual scene, and thus more aligned captions. 

\textbf{Discourse relations.} Rhetorical structure theory studies how text is structured for cohesion \cite{Mann1988RhetoricalST}. 
%There is an argument or a claim (nucleus) which is furthered by supporting spans (satellite) through a particular type of relation. 
In the supplementary materials, we show the biggest difference in coherence relations occurs for ``Elaboration" (10.5\% more in DII than SIS) and ``Attribution" (3.5\% more in SIS).
%, ``Joint" (1.9\% more in SIS) and ``Enablement" (1.7\% more in SIS) relations. Labels extracted from Temporal-SIS captions could contain either a future or past (``before'', not currently visible) reference in nucleus/satellite; while Temporal-DII contains references to the present (``while''). 

\textbf{Visual-text alignment.} The average cosine similarity over DII caption-image embeddings extracted using CLIP \cite{Radford2021LearningTV} is $0.3032\pm0.0345$, significantly larger than for SIS, $0.2633\pm0.0450$. 
In our supplementary materials, we show SIS exhibits more diverse image-text relations (CLUE discourse types \cite{Alikhani2020ClueCC}) than DII.

\subsection{Descriptiveness features and predictor}

%\input{iccv2023AuthorKit/tables/dii_sis_classifier_table.tex}
\input{iccv2023AuthorKit/tables/dii_sis_clsf.tex}

Based on the above analysis, we examine \textbf{which linguistic features are most discriminative} between descriptive and narrative captions. We assign a positive label to captions drawn from the DII split and a negative label to SIS captions. The input vector to this classifier contains binary variables corresponding to the presence of a linguistic feature (e.g. proper noun, adjective, verb - past tense, etc) in the caption. 
We compare different combinations of the input in table \ref{tab:dii_sis_classifier}.
We find that part-of-speech is the strongest linguistic feature, and performs nearly as well as BERT \cite{BERT}, despite being much smaller and having less overhead (no forward pass required). 


\subsection{Descriptiveness ratio in in-the-wild datasets}
%\textbf{How well does this classifier transfer to other in-the-wild datasets?}

%\input{iccv2023AuthorKit/tables/descriptiveness_performance.tex}

We label 100 captions in each of SBUCaps, RedCaps, Conceptual Captions and COCO, as having a descriptive or narrative style. We define ``descriptive'' style as the caption describing important parts of the image and using objective language. We define ``narrative'' as having subjective elements, first-person perspective ("I", "my", etc), using non-literal expressions ("it's a piece of cake"), or assigning intent ("owner shows off her dog"). While our criteria are based on VIST-SIS, they are inclusive of captions beyond those narrative examples.
%, as real-world captions are not constrained by creating a caption drawing from visible events in previous or future frames. 
%We find that in-the-wild datasets contain far more narrative-like examples than COCO, a heavily descriptive dataset as shown in Table \ref{tab:descriptiveness_in_wild_annot}. 
We found RedCaps contains the most narrative-like captions (62\%), SBUCaps contains 37\%, and ConceptualCaptions 33\% (lowest amongst in-the-wild datasets), and COCO had 5\%. 
This is understandable because RedCaps are from a social media source, where people frequently write in a story-like fashion to communicate and connect with others; contrastively, Conceptual Captions is written with the intent to convey the image, or sometimes the meaning behind the image to visually impaired users using assistive technology. 
%we show the ability of our descriptiveness classifier to transfer to these datasets. 
%In fact, it's surprising that there's still a considerable amount of narrative-like captions in a heavily preprocessed image-alt text dataset like Conceptual Captions.
%Next, we test the ability of the part-of-speech based descriptiveness classifier trained on VIST descriptive and narrative captions to predict whether an in-the-wild caption is descriptive. We use the small subset mentioned earlier for evaluation.
In our supplementary materials, we show that while our part-of-speech descriptiveness classifier is able to correctly identify descriptive captions in most datasets, it struggles with correctly identifying narrative captions. 
%We suspect that this might be due to the domain shift from VIST-SIS to the narratives found in the real world. Furthermore, the features that indicate narrativeness in the natural captions are not represented by part-of-speech features. 
For example, "interesting" (an adjective) indicates subjectivity, but "red" (also adjective) is concrete. 
%first-person pronouns like "I" and "my" fall under personal pronouns. 
%But, beyond the part of speech tags, there are implicit first-person perspectives found in the grammatically incorrect short hand writing found in natural captions: "watching a doggie show in the bar while waiting for the pizza". The underspecification of the features used for the descriptiveness classifier explains why it fails to generalize to narrative captions in-the-wild.


This motivates our VEIL approach which extracts broader patterns than those studied in this section.




==> iccv2023AuthorKit/old_files/method.tex <==
\section{Methods}
\subsection{Extracting Labels}
\label{sec:extracting}

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.30]{iccv2023AuthorKit/figures/images/wsod_model_diagram.drawio.png}
    \caption{Diagram explaining global and local view considerations while extracting labels from captions. The local view classifier takes \textbf{a} feature among: gerund, verb base form, past tense, past participle, non-3rd person singular present, 3rd person singular present, nucleus, satellite, subject, object.}
    \label{fig:global_local}
\end{figure}

\textbf{DII/SIS Classifier}
In our previous analysis, we observed that linguistic features like part of speech and discourse relations like RST \cite{Mann1988RhetoricalST} 
and CLUE \cite{Alikhani_Stone_2019} 
are distinctive between descriptive and narrative captions. We train a logistic regression classifier to predict the %source of captions (i.e. DII or SIS), or specifically the 
descriptive-ness of the caption. 
%Details of how each caption is tagged with linguistic features is mentioned in Section 3.
%We extract Part-of-Speech tags using SpaCy, a natural language processing library \cite{spacy2}. We extract RST discourse relations in two stage approach. First, we segment the caption into elementary discourse units using the method described in Li et al. \cite{li_segbot} and then use an off-the-shelf model \cite{wang-etal-2017-two} to produce an RST diagram. Discourse relations corresponding to each caption are then extracted from the RST diagram.

\noindent \textbf{Rule Based Classifier}
The global view method, described above, filters out entire captions. The local view method, on the other hand, chooses to extract labels based a lexical match between the selected categories and a five-word window of a particular linguistic feature in a caption. We illustrate this in Fig.~\ref{fig:global_local}. For nucleus/satellite local view classifiers, lexical match is directly applied to the span associated with nucleus or satellite, rather than a 5-word window.

\subsection{Weakly Supervised Object Detection}
\label{sec:wsod}

We follow prior literature \cite{bilen2016weakly,Ye_Zhang_Kovashka_Li_Qin_Berent_2019} to train a network to predict the labels identified in Sec.~\ref{sec:extracting}.
A convolutional neural network base encoder $h(x_i)$ is used to extract a feature map for an image, $x_i$. We use VGG-16 \cite{Liu2015VeryDC} with the fully connected layers removed as our base encoder, initialized with pre-trained ImageNet \cite{Deng2009ImageNetAL} weights. Region of interest (ROI) pooling \cite{Girshick2015FastR} is then applied to the feature map and the regions of interest $R_i \in \mathbb{R}^{4\times M}$ to generate a feature embedding $\phi(x_i)_m$ for each region: 
$\phi(x_i) = ROIPool(h(x_i), R_i)$.
We initialize two parallel fully-connected layers $f_c$ and $f_d$ whose outputs will be normalized to give a classification score, the probability that an object $c$ is present in that region, and detection score, the probability that $R_{i,m}$ contributes to the image-level class prediction, respectively. 
\begin{equation}
    p^{cls}_{m, c} = \sigma{(f_c(\phi(x_i)_m))}, ~~~ p^{det}_{m, c }=\frac{\exp\Big(f_d(\phi(x_i)_m)\Big)}{\sum_{j=1}^{M} \exp\Big(f_d(\phi(x_i)_j)\Big)}
\end{equation}

The class and detection predictions for each region are multiplied and summed over $M$ proposals to produce one image-level class prediction vector.
\begin{equation}
    \hat{p_c}=\sigma\Bigg(\sum_{m=1}^{M} p_{m,c}^{det} o_{m,c}^{cls}\Bigg)    
\end{equation}  

To train, we apply the multiple instance detection loss to the extracted image-level label and the predicted image-level label \cite{bilen2016weakly}:
\begin{equation}
    L_{mid}=\frac{1}{C}\sum_{c=1}^{C}\Big[y_c \log \hat{p_c} + (1 - y_c) \log(1-\hat{p_c})\Big]
\end{equation}



==> iccv2023AuthorKit/old_files/old_cross_category.tex <==
% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c}


% bicycle
% bird
% boat
% bus
% dining table
% horse
% person
% all
% Counts of VPELs
% 329
% 300
% 295
% 168
% 207
% 277
% 297
% 1873
% VPEL Detection PREC/REC/F1
% unfiltered
% 0.651/1.000
% 0.789
% 0.549/1.000
% 0.709
% 0.544/1.000
% 0.705
% 0.241/1.000
% 0.388
% 0.413/1.000
% 0.585
% 0.531/1.000
% 0.693
% 0.546/1.000
% 0.706
% 0.486/1.000
% 0.654
% Ood filtered
% 0.753/0.362
% 0.489


% 0.805/0.440
% 0.569
% 0.821/0.451
% 0.582
% 0.423/0.393
% 0.407
% 0.676/0.604
% 0.638
% 0.755/0.791
% 0.772
% 0.719/0.535
% 0.614
% 0.713/0.509
% 0.594


% Id filtered
% 0.774/0.774
% 0.774
% 0.738/0.760
% 0.749
% 0.694/0.729
% 0.711
% 0.701/0.405
% 0.513
% 0.533/0.657
% 0.589
% 0.734/0.798
% 0.765



% 0.66/0.714
% 0.686
% 0.693/0.701
% 0.697


%     \end{tabular}
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table}
% % % % % % % %  ON ALL ID CATEGORIES, OLD RUN %%%%%%
% \begin{table}[]
%     \centering
%     \begin{tabular}{|c|p{30}|p{25}|c|c|}\hline
% Method & Masking Prob. & Special Token & Prec/Rec & F1 \\\hline
% unfiltered & 0.00 & \xmark & 0.428 / 1.000 & 0.599 \\\hline
% ID & 0.00 & \xmark & 0.720 / 0.687 & 0.703 \\\hline
% OOD & 0.00 & \xmark & 0.745 / 0.321 & 0.448 \\\hline
% OOD & 0.25 & \xmark & 0.712 / 0.447 & 0.549 \\\hline
% OOD & 0.00 & \checkmark & 0.746 / 0.468 & 0.575 \\\hline
%     \end{tabular}
%     \caption{The use of a special token for predictions significantly improves recall. This could mean that this setup decreases the category-specific dependency of determining whether an object mention is noisy.}
%     \label{tab:cross_category}
% \end{table}

==> iccv2023AuthorKit/old_files/old_direct_eval_file.tex <==
\begin{table*}[h]
\begin{center}
\begin{tabular}{|>{\centering\arraybackslash}m{0.75in}|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{} & \multicolumn{1}{|c|}{} & \multicolumn{2}{|c|}{\textbf{SBUCaps}} & \multicolumn{2}{|c|}{\textbf{RedCaps}} & \multicolumn{2}{|c|}{\textbf{Conceptual Captions}} \\\cline{2-8}
 & \textbf{Method} & \textbf{PREC / REC} & \textbf{F1} & \textbf{PREC / REC} & \textbf{F1} & \textbf{PREC / REC} & \textbf{F1} \\
\cline{2-8}
& No filtering & 0.463 / 1.000 & 0.633 & 0.596 / 1.000 &  0.747 & 0.737 / 1.000  & \underline{0.849} \\
\hline
\multirow{2}{*}{\makecell{Image + Lang. \\ Conditioned}}&Global CLIP \cite{Radford2021LearningTV} & 0.531 / 0.700 & 0.604 & 0.618 / 0.551 & 0.583 & 0.753 / 0.458 & 0.569 \\
& Global CLIP - E \cite{Radford2021LearningTV} & 0.526 / 0.683 & 0.594 & 0.625 / 0.522 & 0.569 & 0.745 / 0.417 & 0.534 \\
 \hline
\multirow{3}{*}{\makecell{ Image \\ Conditioned}}&   Local CLIP \cite{Radford2021LearningTV} & 0.588 / 0.246 &  0.347 & 0.723 / 0.591 & 0.651 & 0.750 / 0.240 & 0.363 \\
& Local CLIP - E \cite{Radford2021LearningTV} & \underline{0.708} / 0.820 & \underline{0.760} & \underline{0.770} / 0.924 & \underline{0.840} & \underline{0.842} / 0.462 & 0.597 \\
& Largest Loss Simulation \cite{Kim2022LargeLM}
 & 0.530 / \underline{0.898} & 0.667 & 0.700 / 0.908 & 0.790 & 0.806 / 0.858 & 0.831 \\
  \hline
\multirow{7}{*}{\makecell{Language \\ Conditioned}}& Descriptiveness Score & 0.449 / 0.542 & 0.491 & 0.561 / 0.326 & 0.413 & 0.739 / 0.741 & 0.740 \\
&Narrativeness Score & 0.482 / 0.458 & 0.470 & 0.619 / 0.674 & 0.645 & 0.738 / 0.259 & 0.383 \\
&Noun modifier-1 (Rule)
 & 0.530 / 0.692 & 0.600 & 0.637 / 0.633 & 0.635 & 0.782 / 0.757 & 0.769 \\
& Noun modifier-2  (Rule)
 & 0.537 / 0.673 & 0.597 & 0.643 / 0.593 & 0.617 & 0.784 / 0.749 & 0.766 \\
 &  Cap2Det \cite{ye_2019_cap2det}
 & 0.500 / 0.884 & 0.639 & 0.633 / \textbf{0.945} & 0.758 & 0.758 / \textbf{0.956} & 0.846 \\\cline{2-8}
& AM Same Dataset
 & \textbf{0.946} / \textbf{0.956} & \textbf{0.951} & \textbf{0.855} / \underline{0.929} & \textbf{0.890} & \textbf{0.922} / \underline{0.955} & \textbf{0.938}\\
& AM Cross-Dataset
 & 0.636 / 0.811 & 0.713 & 0.747 / 0.847 & 0.793 & 0.832 / 0.824 & 0.828\\
\hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{|p{3cm}|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{\textbf{}} & \multicolumn{2}{|c|}{\textbf{COCO}} & \multicolumn{2}{|c|}{\textbf{VIST}} & \multicolumn{2}{|c|}{\textbf{VIST-DII}} & \multicolumn{2}{|c|}{\textbf{VIST-SIS}} \\
\hline
\textbf{Method}  & \textbf{PREC / REC} & \textbf{F1} & \textbf{PREC / REC} & \textbf{F1}  & \textbf{PREC / REC} & \textbf{F1}  & \textbf{PREC / REC} & \textbf{F1} \\
\hline
No filtering & 0.948 / 1.000 & 0.973 & 0.744 / 1.000 & 0.853 & 0.779 / 1.000 & 0.876 & 0.695 / 1.000 & 0.820\\ \hline
G CLIPScore & 0.945 / 0.509 & 0.662 & 0.772 / 0.589 & 0.668  & 0.788 / 0.518 & 0.625 & 0.754 / 0.624 & 0.683 \\
E - G CLIPScore & 0.931 / 0.487 &  0.640 & 0.769 / 0.569 & 0.654 & 0.785 / 0.504 &  0.613 & 0.741 / 0.595 & 0.660 \\
LV CLIPScore & 0.951 / 0.307 & 0.464 & 0.752 / 0.298 & 0.427 & 0.787 / 0.341 & 0.476 & 0.738 / 0.292 & 0.418 \\
E - LV CLIPScore & 0.972 / 0.663 & 0.788 & 0.874 / 0.671 &  0.759  & 0.886 / 0.572 & 0.695 & 0.833 / 0.793 & 0.812\\ \hline
Desc. Score &  0.948 / 0.923 & 0.935 & 0.755 / 0.631 & 0.687 & 0.784 / 0.913 & 0.844 & 0.686 / 0.163 & 0.264\\
Narr. Score & 0.942 / 0.077 & 0.143 & 0.717 / 0.369 & 0.487 & 0.697 / 0.087 & 0.154 &  0.691 / 0.837 & 0.757 \\
Rule 1 & 0.963 / 0.666 & 0.788 & 0.777 / 0.839 & 0.807 & 0.814 / 0.828 & 0.821 & 0.717 / 0.863 & 0.783 \\
Rule 2 & 0.964 / 0.656 & 0.781 & 0.780 / 0.832 & 0.805 & 0.814 / 0.819 & 0.817 & 0.719 / 0.846 & 0.777 \\ \hline
Cap2Det & Cell 8 & Cell 9 & Cell 10 & Cell 11 & Cell 8 & Cell 9 & Cell 10 & Cell 11\\ \hline
LLM Simulation & Cell 8 & Cell 9 & Cell 10 & Cell 11 & Cell 8 & Cell 9 & Cell 10 & Cell 11 \\ \hline
AM Same Dataset & 0.948 / 1.000 & 0.973 & 0.789 / 0.971 & 0.871 & 0.819 / 0.992 & 0.892 & 0.690 / 0.998 & 0.816 \\
AM Cross-Dataset & 0.975 / 0.942 & 0.958 & 0.835 / 0.920 & 0.875 & Cell 8 & Cell 9 & Cell 10 & Cell 11 \\

\hline
\end{tabular}
\end{center}
\caption{VPEL Detection Evaluation Metrics. While the in domain alignment model (trained on the corresponding train split of the test split) is the highest in terms of F1 score, the largest loss simulation has the highest precision across the three in-the-wild datasets. Selection based on ENSEMBLE - Local view CLIPScore is alo fairly competitive, achieving the second highest REC/F1 in SBUCaps and RedCaps. In terms of descriptiveness, on VIST }
\label{tab:table2_label}
\end{table*}

\hline


==> iccv2023AuthorKit/old_files/old_intro.tex <==
Recent progress in self-supervised and weakly-supervised computer vision tasks has been fueled by data freely available on the web \cite{Radford2021LearningTV,wslimageseccv2018,Jia2021ScalingUV}.  Generally, weak semantic information about visual content is extracted from co-occurring text for a range of tasks from image recognition to weakly supervised object detection to vision-language grounding. Such metadata could come from user-generated content (e.g. tagging, captions) which are constructed by users to serve their own purposes, rather than constructed for pay. This marks a divide between captions written by human annotators following objective guidelines, and how people gravitate towards narratives when creating content, whether it is a caption for a photo posted on Instagram or a voice-over accompanying a documentary. 
Yet weakly supervised object detection (WSOD) methods have been supported \emph{not} by such narrative data, but by crowdsourced, paid-for datasets such as COCO and Flickr30K. Not only are these datasets of a limited scale, but the captions in these datasets often take on only descriptive styles \cite{huang2016visual}. Furthermore, they do not represent the full diversity of written language due to annotation instructions \cite{Alikhani_Stone_2019}. 

Language supervised approaches are only a proof of concept when applied to small datasets. Its potential to match and/or exceed fully-supervised methods appears when it can harness large amounts of data \cite{Jia2021ScalingUV, Radford2021LearningTV, wslimageseccv2018}. Not only has weakly supervised object detection not been applied to large-scale internet data, but there are various challenges to using such data for WSOD; training resources (WSOD has a higher memory usage than weakly supervised image recognition), extracted label noise (objects in the image missing from caption, or objects mentioned in the caption but not in the image), and diverse images (could contain a lot of atypical object instances). We attempt to take a deeper look at applying WSOD to in-the-wild data and applying existing label noise detection and correction.

Motivated by the difference between in-the-wild captions and constructed-for-pay captions, we first verify the linguistic differences between descriptive and subjective narrative styles on an existing image-caption dataset \cite{huang2016visual} with explicitly labeled descriptive and narrative captions. We hypothesize that descriptive captions are cleaner than narrative captions. We use discriminative linguistic features to construct a descriptiveness score predictor which is applied to other in-the-wild image-caption datasets, such as RedCaps \cite{Desai2021RedCapsWI}, SBUCaps \cite{Ordonez2011Im2TextDI}, and ConceptualCaptions \cite{Sharma2018ConceptualCA}, to filter out narrative captions.
\begin{figure}
    \centering
    \includegraphics[scale=0.25]{iccv2023AuthorKit/figures/images/vael_examples.png}
    \caption{\textbf{Examples of types of visually absent extracted labels (VAELs).} In-the-wild captions, depending on the source have varying types of visually absent mentioned objects in their captions. Each of these type of VAELs, signifies the importance of semantic context implied by the rest of the caption when choosing to extract the label.}
    \label{fig:vael_examples}
\end{figure}

Label noise falls into two categories: objects that appear in the image but are not mentioned in the caption and objects mentioned in the caption but don't appear in the image. The first type of noise is intuitive to understand; there are many objects that appear in the image, but not all are worth writing about (background or objects not relevant to the plot). However, the second type of noise is a little strange; after all, why would an object be mentioned if it doesn't appear in the image? This can be explained by how image-level labels are obtained from captions. Since labels are extracted based on exact match (ignoring any punctuation) with a predefined label set, there may be different senses that are used or the extracted label is related to another word (class label bolded; ``hot \textbf{dog}", ``\textbf{car} park") which may or may not be related to the class label's word sense. Additionally, the mentioned object may be a narrative artifact, and it may be implied in the caption that the object is not present as shown in Figure \ref{fig:vael_examples}. These different types of VAEL motivates considering the semantics before deciding to extract a label.

Label noise from object mentions in captions, can follow a visual pattern. The visually absent object mention (bus in ``We were waiting for the bus at the bus stop") can appear in similar visual contexts (bus stop) or the use of two similar (but distinct) objects classes interchange-ably  like mentioning “car” instead of “truck”. Additionally, polysemic object names would have visual neighbors with the same label, but not the same sense as class labels defined by object detection datasets. For example, “bed” could be a bed for a dog or bed for a human or an ``explicitly" noisy sense ``bed” w.r.t. a garden. This type of structured false positive noise is harmful for a precise localization task, like object detection as it may increase dependence on contextual cues. Empirically, we show that language-agnostic data-dependent noise correction approaches that appear to be robust to structured noise in image recognition (benefits from contextual cues), show limited improvements in localization when compared to language-conditioned noise filtering approaches.

Ultimately, we conduct an exploratory study of types of noises across diverse datasets and compare language-conditioned methods and language-agnostic noisy label detection to identify noisy labels. Specifically, our contributions are as follows:
\begin{itemize}
    \item Develop a taxonomy of image-level label noise found in in-the-wild captions.
    \item Illustrate narrative-like tendencies and other differences in linguistic structure of in-the-wild captions compared to descriptive captions.
    \item Apply and compare both new language-conditioned and existing language-agnostic label noise detection/correction approaches across constructed-for-pay image caption datasets \cite{huang2016visual, Lin2014MicrosoftCC} and a wide set of in-the-wild datasets that span sources the following: social media \cite{Desai2021RedCapsWI}, photo-sharing platform \cite{Ordonez2011Im2TextDI}, and image-alt-text pairs \cite{Sharma2018ConceptualCA}.
    \item Evaluate label noise correction techniques in their ability to correctly detect label noise and their performance on benchmarks.
    \item Our transformer-based extracted label, visual presence classifier (object-alignment model) performs better than all other label noise correction techniques in recognizing visually present extracted labels and when used to filter labels for weakly supervised object detection. The resulting object detection model shows substantial improvements on common object detection benchmarks \cite{Everingham2010ThePV, Lin2014MicrosoftCC}.
\end{itemize}





% ----- OLD TEXT

%Specifically, for the task of weakly supervised object detection, we want to determine if a mentioned object in the caption should be extracted as a label. Language provides additional context that may indicate that the mentioned object in the caption might not be visible in the corresponding image. We compare against using existing methods such as CLIP, or a simple baseline to identify this misalignment or can other language-structure conditioned heuristics perform better? We compare these methods across a wide set of in-the-wild datasets that span sources the following: social media \cite{Desai2021RedCapsWI}, photo-sharing platform \cite{Ordonez2011Im2TextDI}, and image-alt-text pairs \cite{Sharma2018ConceptualCA}. In addition to the language-conditioned approaches mentioned earlier, we compare against existing language-agnostic noisy multi-label classification techniques. These methods typically rely on the assumption that clean labels have simpler patterns that are learnt earlier in training and this knowledge can be exploited later in training. However, this either assumes that noise is weak or unstructured. Label noise from object mentions in captions, have a pattern. The visually absent object mention (bus in "We were waiting for the bus at the bus stop") can appear in similar visual contexts (bus stop) or the use of two similar (but distinct) objects classes interchange-ably  like mentioning “car” instead of “truck”. Additionally, polysemic object names would have visual neighbors with the same label, but not the same sense as object detection datasets. For example, “bed” could be a bed for a dog or bed for a human, but object detection datasets have a higher representation of the latter or an explicitly noisy sense “bed” w.r.t. a garden.  Empirically we find that the language-agnostic noisy label selection and/or correction approaches perform better than unfiltered baselines, they still have limited improvement in object localization, as opposed to object recognition, due to the structured noise. 

%The use of in-the-wild multimodal data (Conceptual Captions) has been mainly limited to tasks like caption generation and image-text or video-text grounding. Larger, diverse data have been sourced from social media like Instagram for weakly supervised image recognition \cite{wslimageseccv2018}; however, image-level labels  are inferred from Instagram hashtags – not user-provided captions. Weakly supervised object detection (also semantic segmentation) approaches have demonstrated the use of extracting labels from descriptive human-annotated captions \cite{ye_2019_cap2det}. 

%Even in vision-language grounding where diverse, noisy multimodal datasets have been used, there appear to be diminishing returns when naively increasing the dataset (by including noisy examples). For example, ALIGN \cite{Jia2021ScalingUV}, trained on 1 billion samples, shows little-to-no improvement over CLIP, trained on 400 million image-text pairs, on finetuned or zero-shot ImageNet, an image recognition benchmark. Image-text grounding from larger image-text datasets such as LAION-5B \cite{Schuhmann2022LAION5BAO} show improvements on less than half of zero-shot image recognition benchmarks despite using 10x more data than CLIP. While there may be other reasons why performance degrades or shows no improvements when using so much more data, one reason might be that there are semantic misalignments within the image and the caption. 



==> iccv2023AuthorKit/old_files/old_vetting_analysis_onCLAN.tex <==
\begin{table*}[h]
\begin{center}
\small    
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
        & \multicolumn{3}{c|}{Label noise} & \multicolumn{2}{c|}{Similar object} & \multicolumn{3}{c|}{Visual defects} & \multicolumn{6}{c|}{Linguistic indicators} \\ \hline
         Vetting Method & {\scriptsize \%Vis} & {\scriptsize \%Part} & {\scriptsize \%Abs} & {\scriptsize \%Co-occ} & {\scriptsize \%Sim} & {\scriptsize \%Occl} & {\scriptsize \%Parts} & {\scriptsize \%Atyp}  & {\scriptsize \%Mod} & {\scriptsize \%Prep}  & {\scriptsize \%Non-lit} & {\scriptsize \%Sense} & {\scriptsize \%Named} & {\scriptsize \%Beyond} \\ \hline
        \multicolumn{15}{|c|}{SBUCaps}\\\hline
        VEIL-Same Dataset & 83.3 & \textbf{85.0} & \textbf{94.7} & \textbf{87.0} & \textbf{80.0} & \textbf{81.1} & \textbf{90.6} & \textbf{87.2} & \textbf{95.2} & \textbf{93.9} & \textbf{90.6} & \textbf{100.0} & \textbf{100.0} & \textbf{88.8} \\ 
        % VEIL-Cross Dataset & 45.2 & 72.3 & 67.5 & 63.7 & 55 & 60.4 & 65.6 & 47.8 & 76.6 & 77.5 & 75.6 & 91.6 & 70.8 & 52.8 \\ \hline
        LocalCLIP-E & 69.0 & 51.5 & 80.7 & 71.3 & 70.0 & 52.7 & 52.1 & 65.6 & 63.8 & 70.6 & 82.9 & 96.2 & 62.5 & 82.4 \\ \hline
        \multicolumn{15}{|c|}{RedCaps}\\\hline
        VEIL-Same Dataset & 63.3 & \textbf{91.7} & 74.1 & \textbf{71.4} & \textbf{85.7} & \textbf{83.3} & \textbf{89.0} & \textbf{68.3} & \textbf{74.8} & \textbf{90.0} & 66.7 & \textbf{88.9} & 80.9 & 76.3 \\ 
        % VEIL-Cross Dataset & 54.1 & 68.3 & 61.5 & 50 & 45.2 & 58.3 & 74.2 & 50 & 69.2 & 63.3 & 33.3 & 72.2 & 71.4 & 60.4 \\ \hline
        LocalCLIP-E & 15.9 & 52.8 & \textbf{78.4} & 40.0 & 38.1 & 47.0 & 45.0 & 23.2 & 68.4 & 63.3 & \textbf{70.8} & \textbf{70.6} & \textbf{90.0} & \textbf{76.7} \\ \hline
        \multicolumn{15}{|c|}{CC}\\\hline
        VEIL-Same Dataset & 58.5 & 60.6 & 83 & 81.2 & 55 & 54.9 & 53.6 & 56.3 & 64.2 & 73.7 & 81.7 & 100 & - & 77.4 \\ 
        % VEIL-Cross Dataset & 61.6 & 42.8 & 64.1 & 67.4 & 45 & 42.2 & 50 & 65.6 & 76.7 & 54 & 63.3 & 87.5 & - & 45.4 \\ \hline
        LocalCLIP-E & 26.2 & 45.0 & 89.1 & 74.9 & 57.5 & 49.9 & 50 & 24.1 & 73.3 & 63.9 & 91.7 & 100.0 & - & 86.8 \\ \hline
    \end{tabular}
    \end{center}
    \caption{Vetting VAEL Recall on CLaN Dataset. Bold indicates best performance in column for each dataset }
    \label{tab:vetting_analysis}
\end{table*}

==> iccv2023AuthorKit/sections/old_text/dump.tex <==
%First, we confirm that the precision of extracted labels from captions from three in-the-wild datasets is far lower than curated, descriptive captions from COCO \cite{Lin2014MicrosoftCC} and VIST-DII \cite{huang2016visual}.

%Building on this, we show that the narrative element found in in-the-wild corpora can impact the ability to successfully train an object detection model, and the contribution of this noise can be reduced using VEIL.
%Multimodal datasets commonly include vision and language data, but differ in the form each modality is presented; for example, the vision modality can be presented via static images \cite{Schuhmann2021LAION400MOD,Radford2021LearningTV,wslimageseccv2018}, images in a sequence \cite{huang2016visual,Yagcioglu2018RecipeQAAC}, or long \cite{Miech2019HowTo100MLA,Chen_2017_CVPR} or short videos \cite{Tang2021ComprehensiveIV}. Similarly, language in multimodal datasets can also be represented in diverse forms such as procedural (instructional) language \cite{Miech2019HowTo100MLA,Yagcioglu2018RecipeQAAC,Hessel2019UnsupervisedDO}, narrative-like language
%\cite{huang2016visual,Chen_2017_CVPR,Biten2019GoodNE,Huang2020MovieNetAH,Thomas2019PredictingTP, Ordonez2011Im2TextDI, Desai2021RedCapsWI}, user-written alternative text \cite{Sharma2018ConceptualCA,Radford2021LearningTV,Lin2014MicrosoftCC,Young2014FromID}.
%Typically, instructional videos have been used for learning visual-textual grounding \cite{Miech2019HowTo100MLA,Miech2020EndtoEndLO}; Hessel \etal \cite{Hessel2020BeyondIV} studied the extension to using \textit{diverse non-instructional videos} for visual-textual grounding. Similarly part of our work studies the effect of \textit{extracting labels} from descriptive or narrative captions for weakly supervised object detection, rather than a multimodal retrieval-based notion of grounding. We also go beyond studying differences in object detection performance when extracting labels from descriptive or narrative captions and generally screen for false positive extracted label noise.

%, prior to finetuning detection using full supervision from a constrained set of classes. 
%As described in detail in the previous section, vision-language pretraining for open vocabulary object detection utilizes captions during pretraining while detection can be learnt from annotated bounding boxes \cite{zareian2021open}.  or from pseudo-labeled bounding boxes \cite{regionclip}. \cite{Gao2021OpenVO} or a combination of both \cite{Li2021GroundedLP_GLIP} uses both ground truth and pseudo-labeled bounding boxes .
%Additionally, we argue that false positives are far more harmful than false negatives, as there are few positive examples than there are negative examples. 
% Another approach used a vision-language dataset during pretraining, and bounding boxes for only some categories, to generalize detection abilities to novel classes \cite{zareian2021open}. 

%Zero-shot detection \cite{ZSOD_1_Bansal_2018_ECCV} is a task that tests the ability of an object detection model trained on a set of base classes to generalize to a set of unseen target classes. 

%Lastly, Detic \cite{Zhou2022DetectingTC} performs weakly supervised object detection with a CLIP-based open vocabulary classifier head on ImageNet \cite{Deng2009ImageNetAL} and Conceptual Captions \cite{Sharma2018ConceptualCA} as pretraining prior to supervised learning from base class examples. 

% some papers:
% Learning to Prompt for Open-Vocabulary Object Detection with Vision-Language Model
% RegionCLIP
% ProposalCLIP
% ECCV 2022 https://arxiv.org/abs/2111.09452 
% Detic
%GLIP

% We evaluate only the state-of-the-art small-loss-based approach \cite{Kim2022LargeLM} on weakly supervised object detection because it's computationally efficient to integrate with WSOD. %Our work is complementary to the progress in this problem because 
%This highlights another area for adaptive noise reduction methods to focus on.

%One could also perform label extraction that considers synonyms, synsets, and word-similarity based matching against a closed vocabulary set; this can significantly increase the number of examples \footnote{For our purposes this is not needed since we are only trying to show that visual presence can be detected directly from captions even while learning from noisy pseudo-visual presence labels and that VEIL's filtering significantly improves WSOD performance compared to no filtering and language agnostic filtering and/or correction.}. 

%We begin with a case study of the VIST dataset \cite{huang2016visual} which contains both descriptive and narrative captions for the same image (presumably cleaner/noisier, respectively). We then examine broader noise patterns extending beyond narrativeness, in three additional datasets. 

% FROM METHOD 

% These embeddings are then passed to BERT, which performs multi-head self-attention over the tokens and outputs token-level output embeddings $v\in \mathbb{R}^{C\times d}$

%This is represented as an indicator function $\mathbbm{1}_{EL}(i)$ in our description below, but in practice is simply a vector mask. 
%(See Table \ref{}). This 250 image-caption subset was annotated with visual presence/absence of certain objects (elephant, truck, cake, bus, cow) for each of the in-the-wild datasets.
%The image and caption's visual presence pseudo labels are represented as binary vector $y$ where 1 denotes visual presence. 
% An extracted label mask with the same length as the number of tokens and all the tokens corresponding to an extracted label is marked as 1. This mask is set up such that the binary cross entropy loss averaged only over the tokens associated within the extracted label token set $EL$.

%with one hidden layer followed by the tanh activation function:

%special token works better empirically in generalizing to new categories in addition to generalizing to other datasets. Overall, we show that these techniques can help improve its ability to generalize to new categories.

% We test out additional variants that reduce the model's reliance on category specific predictions: inserting a special token right before each extracted label and randomly masking the tokens associated with the extracted labels with probability $p_m$. We hypothesize that a special token can learn a representation specific to vetting, rather than   There are other existing special tokens like {\tt [CLS], [SEP], [MASK] } in BERT \cite{BERT}; so we add {\tt [EM\_LABEL] } to the vocabulary and its respective fixed input embedding is randomly initialized. When preprocessing the caption, this special token is injected before the object mention within the caption. The model should be able to implicitly learn that this token is related to the adjacent tokens through positional embeddings concatenated with each input embedding, an existing feature of transformers \cite{Attn_Vaswani}. 

% We ignore predictions from tokens not associated with an extracted label, but these tokens are useful in establishing caption context. 
% MOVING PART ABOUT GOLD/PSEUDO GROUND TRUTH LABELS TO ANALYSIS SECTION

% We follow prior literature \cite{bilen2016weakly,Ye_Zhang_Kovashka_Li_Qin_Berent_2019} 
% to train a network to predict object categories.
% A convolutional neural network base encoder $h(x_i)$ is used to extract a feature map for an image, $x_i$. We use VGG-16 \cite{Liu2015VeryDC} with the fully connected layers removed as our base encoder, initialized with pre-trained ImageNet \cite{Deng2009ImageNetAL} weights. Region of interest (ROI) pooling \cite{Girshick2015FastR} is then applied to the feature map and the regions of interest $R_i \in \mathbb{R}^{4\times M}$ to generate a feature embedding $\phi(x_i)_m$ for each region: 
% $\phi(x_i) = ROIPool(h(x_i), R_i)$.
% We initialize two parallel fully-connected layers $f_c$ and $f_d$ whose outputs will be normalized to give a classification score, the probability that an object $c$ is present in that region, and detection score, the probability that $R_{i,m}$ contributes to the image-level class prediction, respectively. 
% \begin{equation}
%     p^{cls}_{m, c} = \sigma{(f_c(\phi(x_i)_m))}, ~~~ p^{det}_{m, c }=\frac{\exp\Big(f_d(\phi(x_i)_m)\Big)}{\sum_{j=1}^{M} \exp\Big(f_d(\phi(x_i)_j)\Big)}
% \end{equation}

% The class and detection predictions for each region are multiplied and summed over $M$ proposals to produce one image-level class prediction vector.
% \begin{equation}
%     \hat{p_c}=\sigma\Bigg(\sum_{m=1}^{M} p_{m,c}^{det} o_{m,c}^{cls}\Bigg)    
% \end{equation}  

% To train, we apply the multiple instance detection loss to the extracted image-level label and the predicted image-level label \cite{bilen2016weakly}:
% \begin{equation}
%     L_{mid}=\frac{1}{C}\sum_{c=1}^{C}\Big[y_c \log \hat{p_c} + (1 - y_c) \log(1-\hat{p_c})\Big]
% \end{equation}

% FROM EXPERIMENTS

%We will also describe the implementation details of other methods we compare against.
%\textbf{Implementation Details for Vetting Methods}

%We evaluate the ability of VEIL and other intuitive approaches to vet extracted labels for visual presence on each data source's test split. First, we establish a simple baseline by examining performance without vetting. Then, we'll compare the vetting methods, which are arranged into three categories: language-conditioned, image-conditioned, and image and language conditioned. Note that VEIL-Same Dataset is the only approach trained on the same source's train split and Large Loss Matters \cite{Kim2022LargeLM} is simulated on the test split. 

% Figure 4 in that paper shows the improvement 
%However, the precision may suggest that LocalCLIP-E sometimes hallucinates an object or the ground truth may be missing an object detection (inaccurate visual presence labels). 
% Since image-based approaches for label vetting work quite well, we also tested how much pseudo-labeled data it would take for VEIL-SBUCaps to do better than the image-based methods. Our results shown in Figure \ref{fig:train_subset} (left) indicate only a small amount (25K) is needed to do better in terms of F1 compared to LLM, but more data (75K) is needed to improve F1 over Local CLIP-E. However, all this data is pseudo-labeled so it does not require any additional cost. 

% \textbf{Localization vs. Recognition.}
% We can see that even though Reject Large Loss and Local CLIP-E have strong vetting results (Table \ref{tab:direct_eval}) they perform poorly in weakly supervised object detection (Table \ref{tab:det_v_recognition}). We hypothesize there might be differences in detection and recognition results, as recognition may benefit from some types of noisy data, such as a specific type of structured noise where context is shared between images with the VAEL and examples of actually containing that category.
% When evaluating the precision of image-level predictions on Pascal VOC 2007 \cite{Everingham2010ThePV}, we observe that Local CLIP-E does do better when it comes to recognition ability (+19\% relative to VEIL-SBUCaps), but significantly worse in detection (-62\% relative to VEIL-SBUCaps). Similarly, we observe only an 8\% drop in recognition performance for Reject Large Loss compared to VEIL-SBUCaps but a 38\% drop in detection. VEIL$_{\text{ST}}$-Redcaps,CC is weaker than VEIL-SBUCaps in vetting SBUCaps data, but has a similar performance drop in both detection and recognition. This indicates VEIL vets out noisy labels harmful to localization, even when trained on different sources, and its accepted labels are better for learning localization.

% \input{iccv2023AuthorKit/figures/structured_noise_qual}

% We show examples in Fig.~\ref{fig:structured_qual} containing correct image-level predictions from the LLM-trained WSOD model and the VEIL-SBUCaps-vetted WSOD model. We show recurring examples across categories where parts of the object (car engine) or background context (water or buildings) are detected as the object by LLM. This appears to be the effect of structured noise in training where labels are applied to images that do not fully contain the object. Related noun phrases from the captions (``\textbf{car} engine", ``\textbf{bus} stop") and prepositional phrases (``on \textbf{boat}", not shown due to space) are specific structured noise types that would share visual contents across images. These parts and contextual image regions are exactly what the LLM WSOD model detects as the object while our method captures the actual object with high confidence.
\input{iccv2023AuthorKit/figures/scale}

%Differences in performance might come from higher or lower prevalence of certain VAEL noise types; for example, RedCaps contains more non-literal narrative artifacts than SBUCaps. 
%However, the main takeaway is that across all datasets precision improves significantly compared to no vetting and F1 performance is competitive and better on noisier datasets (improvement in terms of precision overcomes drop in recall). 
%Even though the labels are cleaner, we may still prefer to have better recall so that we can utilize as much data as possible from these datasets. 

%VEIL$_{\text{ST}}$ and random masking the extracted label tokens in the caption. 

% \textbf{Connection to WSOD.}
% To see if precision plays a larger role and can make up for a lower F1 (compared to no vetting) we train MIST \cite{ren2020instance} on the ID test split and compare between no vetting, VEIL-ID and VEIL$_{\text{ST}}$-OOD. In Figure \ref{fig:train_subset} (right), we show that applying VEIL to unseen categories improves performance by . This shows the promise of applying VEIL across category boundaries.
% \textbf{NEED TO CHECK AFTER RESULTS FROM NO VETTING on ID ARE IN - We also used the data from this experiment to compute a correlation between ELV precision/recall, and WSOD mAP results. The only statistically significant correlation we found was for ELV precision and mAP in the OOD setting (but not for recall and mAP), confirming in yet another way the importance of studying precision of extracted labels and VAEL noise.}











% ---------- EVEN OLDER TEXT

%, as well as \cite{tang2017multiple,yang2019towards,zeng2019wsod2,ren2020instance,shen2020uwsod} which iteratively update pseudo-labels based on high-scoring proposals.

% Empirically we find that the language-agnostic noisy label selection and/or correction approaches perform better than unfiltered baselines, they still have limited improvement in object localization, as opposed to object recognition, due to the structured noise. 
%In this paper we want to understand the different types of noise or misalignments that may occur in diverse multimodal datasets on the object or caption level. We develop a taxonomy of noisy labels extracted or not extracted from captions. We find that while some of these seasons may have simple linguistic structural heuristics, others rely more on the surrounding semantic context.

%The only exception is \cite{Chen_2017_CVPR} which uses wildlife documentaries but relies on track information, which is available in video but not image datasets. 

% \textbf{Coherence analysis in language and across modalities.} Discourse structure relays syntactic information about how text is organized. In language, each span is connected in a meaningful and coherent manner to the next; \textit{how} it is connected is known as the discourse or coherence relation. Discourse relations and structure are a well studied topic
% %with competing theories 
% \cite{Mann1988RhetoricalST,webberJoshiDiscourse,wolfGibsonDiscourse}. We use parsers that follow the taxonomy of discourse relations from rhetorical structure theory \cite{Mann1988RhetoricalST}; each span serves a function in rhetoric. This concept was extended to multimodal discourse, specifically images and captions in instructional \cite{Alikhani2019CITEAC} and caption generation contexts \cite{Alikhani2020ClueCC}, but has not been used for object detection before.

%\subsection{Extracted Label Vetting Method}

%There are two variants to the visual presence detection methods. The first produces a single visual presence prediction for the entire caption and the other produces a visual presence prediction \textit{per label}. For the former, the visual presence detection method takes in some text input $t_i$ gathered from the caption $c_i$ for image $x_i$, and produces a score $r_i$. To get a visual presence classification $\hat{y_i}$, the score $r_i$ must be above some threshold. If $\hat{y_i}=1$ then the extracted labels from the caption are accepted, else rejected.

% \textbf{Descriptiveness Classifier.}
% The descriptiveness classifier first computes a frequency-based vector representation of part of speech from $c_i$. Then, this vector $v_i$ is fed as input to a logistic regression model:
% $$\text{descriptiveness\_score} = \sigma(W^Tv_i)$$
% $$\hat{y_i} = \text{descriptiveness\_score} > thresh$$
% The narrativeness score is complementary to the descriptiveness score: $$\text{narrativeness\_score}=1-\text{descriptiveness\_score}$$
% Additionally, for the descriptiveness or narrativeness classifier we set $thresh = 0.5$.


==> iccv2023AuthorKit/sections/old_text/in_the_wild_take2.tex <==
\section{Analysis: Descriptive vs In-the-wild captions}
\label{sec:analysis}

We analyze what makes three large-scale in-the-wild datasets a challenging source of labels for object detection methods.
We begin with a case study of the VIST dataset \cite{huang2016visual} which contains both descriptive and narrative captions for the same image (presumably cleaner/noisier, respectively). We then examine broader noise patterns extending beyond narrativeness, in three additional datasets. 

\subsection{Datasets Analysed}
\label{sec:datasets}

\textbf{COCO} \cite{Lin2014MicrosoftCC} contains cleanly crowdsourced captions, and stands in for the status quo in weakly supervised object detection since the cost of collecting COCO does not scale well.
Visual Storytelling (\textbf{VIST}) \cite{huang2016visual} contains three styles of captions, of which we use two: \textbf{D}escriptions of \textbf{I}mages in \textbf{I}solation (DII), which are similar to COCO captions, 
%commonly used for pretraining for object detection \cite{Lin2014MicrosoftCC,Young2014Flicker30K}, 
and \textbf{S}tory for \textbf{I}mages in \textbf{S}equence (SIS), similar to in-the-wild captions. 
Each image contains both DII and SIS captions, which allows us to observe the impact of caption style while keeping the image constant.
Conceptual Captions (\textbf{CC}) \cite{Sharma2018ConceptualCA}, and the remaining two datasets, are collected from in-the-wild data sources. CC contains 3 million image-alt-text pairs after heavy post-processing; named entities in captions were hypernymized and image-text pairs were accepted if there was an overlap between Google Cloud Vision API class predictions and the caption.
\textbf{RedCaps} \cite{Desai2021RedCapsWI} is the largest dataset used in our paper, consisting of 12M image-text pairs collected from Reddit by crawling a manually curated list of subreddits with heavy visual content.
SBU Captioned Photo Dataset (\textbf{SBUCaps}) \cite{Ordonez2011Im2TextDI} consists of 1 million Flickr photos with associated text descriptions written by their owners.
%on the photo-sharing platform. 
%To construct this dataset, 
Only captions with at least one prepositional phrase and at least 2 matches with a predefined vocabulary were accepted.

The in-the-wild datasets exhibit very low precision of the extracted labels. The precision ranges from 0.463 for SBUCaps, 0.596 for RedCaps, to 0.737 for Conceptual Captions, all much lower than the 0.948 for COCO. This motivates our exploration of VAEL noise.

\subsection{Case Study: Descriptiveness/Narrativeness}
\label{sec:ling_diffs}

% To begin our analysis, 
We use VIST, which contains caption annotations that could be considered a proxy for the quality of labels that could be extracted from corresponding captions. We consider descriptive captions to contain higher-quality labels than narrative captions. We examine some linguistic differences between those captions and then examine the ratio of descriptiveness vs narrativeness in the in-the-wild datasets. We also compare how the descriptive-vs-narrative distinction relates to visual-text alignment. We show that while useful for distinguishing aligned and misaligned images and text on VIST, this distinction is insufficient on other datasets. In Sec.~\ref{sec:expts}, we also show that a descriptiveness classifier does not perform competitively to other techniques for vetting.  This observation means that there are many different types of label noise beyond narrativeness, and we categorize them in a taxonomy, in Sec.~\ref{sec:taxonomy}. It also motivates our development of a technique that can capture broader types of label noise, namely VEIL (Sec.~\ref{sec:veil}).

\textbf{Part of Speech (POS) differences.}
We extract POS tags over all VIST captions using SpaCy \cite{spacy2} and observe differences in pronoun usage and verb tense between descriptive and narrative captions. The increased use of pronouns in SIS suggests a deviation from an impersonal, objective tone. For the same image, one SIS caption says ``\textbf{we} finally arrive at the island" while a DII caption provides count and detailed information: ``\textbf{a group of four men} sitting together".
We also find that present verb tense is much more common in descriptive captions (81\% in DII vs 47\% in SIS) while past tense is more common in narrative captions (19\% in DII and 53\% in SIS). 
DII contains mostly progressive captions (95\%) meaning that it describes ongoing activities more likely to be present in the accompanying visual scene, and thus captions are more visually aligned. Nouns and prepositions are also much more common in DII than SIS. 
In the supplementary file, we show further details about the linguistic distinctions in descriptive and narrative captions.

\input{iccv2023AuthorKit/tables/clip_in_the_wild}

\textbf{Descriptiveness ratio in in-the-wild datasets.}
We label 100 captions in each of SBUCaps, RedCaps, Conceptual Captions and COCO, as having a descriptive or narrative style. We define ``descriptive'' style as the caption describing important parts of the image and using objective language. We define ``narrative'' as having subjective elements, first-person perspective (``I", ``my", etc), using non-literal expressions (``it's a piece of cake"), or assigning intent (``owner shows off her dog"). While our criteria are based on VIST-SIS, they are inclusive of captions beyond those narrative examples.
We found RedCaps contains the most narrative-like captions (62\%), SBUCaps contains 37\%, and CC has 33\% (lowest amongst in-the-wild datasets), and COCO has 5\%. 
This is understandable because RedCaps is from a social media source, where people write in a story-like fashion to communicate and connect with others. In contrast, Conceptual Captions aim to convey the image via a description to visually impaired users. 

While narrativeness is certainly present in these in-the-wild datasets, clean/noisy data need not perfectly align to descriptiveness/narrativeness. We thus assess if the descriptiveness/narrativeness proxy is useful on these in-the-wild datasets by measuring statistics on visual-text alignment. We observe in Table \ref{tab:clip_in_the_wild} that descriptive and narrative captions in VIST are well-separated in terms of alignment. Descriptive captions in SBUCaps, RedCaps, and Conceptual Captions have slightly higher visual-text alignment than narrative ones, but the gap is reduced and is only significant 
on RedCaps (p=0.05). This implies that factors beyond descriptive or narrative drive lower visual-text alignment in these datasets.
%We then test our part-of-speech descriptiveness classifier and show that this classifier has higher precision on descriptive captions in most datasets except RedCaps in our supplementary materials; however, it struggles with correctly identifying narrative captions. 
%Part-of-speech may not fully capture the narrative criteria in our annotation protocol. For example, ``interesting" (an adjective) indicates subjectivity, but ``red" (also adjective) is concrete. 
%Despite these limitations, we still employ the descriptiveness classifier as a vetting baseline. 
This issue has motivated us to investigate label noise in both descriptive and narrative captions more directly, and propose VEIL, which extracts more comprehensive patterns of noise.
%, as described in the following section.


==> iccv2023AuthorKit/sections/old_text/label_noise_taxonomy.tex <==
\subsection{Broader Label Noise Patterns}
\label{sec:taxonomy}

\input{iccv2023AuthorKit/figures/label_taxonomy}

%Objects mentioned in human-annotated captions are usually present in the image (see precision on COCO and VIST-DII in supp.); however, real world captions contain a range of expressions that mention objects not shown in the corresponding image. 
We have identified a taxonomy of label noise found in in-the-wild captions, illustrated in Figure \ref{fig:label_noise_taxonomy}. We focus on 
%with reasons as children nodes for each broad category of noise: 
visually absent, extracted labels (VAELs).
%and visually present, extracted labels (VPEL), with the former being our focus.
%Mentions that are completely missing will now be referred to as visually absent extracted labels (VPELs) and are the main focus of this paper. 
We find that both descriptive and narrative captions mention objects that are semantically unrelated to the category label. 
They can be part of a larger named entity e.g. ``Super \textbf{Bowl} Party" or part of a noun phrase which can either be related to the category e.g. ``\textbf{bottle} opener", or unrelated e.g. ``hot \textbf{dog}" or ``\textbf{orange}'' the color instead of the fruit. Other VAELs are narrative artifacts providing personal context for the image and representing the colorful ways people express themselves. These include non-literal mentions (metaphors and similies), prepositional phrases e.g. ``Left a lighter in my \textbf{car}", describing the past e.g. ``My chest hurts and I can't stop crying. Hugo was run over by a \textbf{car} yesterday", or rarer, negations e.g. ``We did not spot a \textbf{tiger} in our safari". We believe these VAELs can be learned implicitly if a transformer-based model is provided with a loose proxy for visual presence or absence labels, motivating VEIL.
%Not all VAEL examples are equally obvious to recognize without an image reference; this is due to ambiguous language that indicates that some object mentions may be missing from the image but its not obvious ("Sometimes there's a \textbf{dog} under the trucks. I'm on the hunt to photograph him and a \textbf{monkey} or too"). In addition, not all objects in an image are recognizable without an caption prior; people tend to post pictures of their pets in costumes which obfuscates what animal it really is. While we don't explore bad examples of objects in this paper, an emergent behaviour of our model is rejecting atypical examples. We leave exploring this to future work.

% --- OLD TEXT

% Hard examples
% While this is not tackled by this paper, captions can also indicate that the extracted labels would correspond to a hard example: deformed objects (cut up/deteriorated/etc), mostly occluded (most key parts are missing from the image), atypical instances (cat dressed up as something else), out of real world domain (like clipart) – hard where key parts of the object are missing, small objects or objects far off in a distance, close ups where key parts are missing. Other examples might be edge cases: food trucks → can decrease the difference between cars and trucks. Although vans are considered a truck with an enclosed cargo space (WordNet).
% Tractor -> a truck, but with only a cab
% So a truck consists of two parts, a cab and/or a cargo, but even if you have only one part then it is a specific instance of a truck
% Old example
% Antique trucks - [“old”, “antique”, “year mentioned”]

% Chat GPT Rewrite
% Objects mentioned in human-annotated captions are usually present in the image; however, real-world captions can describe a wide range of expressions that may mention objects that are not shown in the corresponding image. In this paper, we focus on a type of label noise called visually absent extracted labels (VPELs), which refers to mentions of objects that are completely missing from the image. There are several reasons why an mentioned object might be visually absent, such as if the object is semantically unrelated to the image or is absent due to narrative artifacts. These semantically unrelated object mentions can be part of a larger named entity, such as "super bowl party," or part of a noun phrase, such as "bottle opener." Other VPELs can be caused by narrative artifacts, such as non-literal mentions (e.g. metaphors and similies), prepositional phrases (e.g. "left a lighter in my car"), descriptions of the past (e.g. "my chest hurts and I can't stop crying. Hugo was run over by a car yesterday"), or negations (e.g. "no tiger"). Additionally, there may be instances that are unrecognizable without the caption, such as objects that are deformed, occluded, atypical, or out of the real-world domain (e.g. clipart).

% It is worth noting that there are also cases where the extracted labels correspond to hard examples, such as objects that are small or far off in the distance, or close-ups where key parts are missing. There may also be edge cases, such as food trucks, which can blur the line between cars and trucks, or tractors, which are considered a specific type of truck. Similarly, antique trucks may be described with words like "old" or "antique" and may include a mention of the year.






==> iccv2023AuthorKit/supp_dump.tex <==
\section{Case Study: Additional Analysis on Descriptiveness/Narrativeness}

\subsection{Linguistic Differences}
Table \ref{tab:pos_dii_sis} presents the distribution of part-of-speech tags in DII and SIS captions, revealing a significant disparity in frequency across various parts of speech. We show that verb tense is more evenly distributed in narrative than descriptive captions which favor present tense. Additionally, Table \ref{tab:aspect} shows aspect, inferred using part-of-speech tags. Aspect relates to visual-text alignment. Progressive aspect refers to verbs that describe an ongoing, hence likely to be shown, activity such as ``The event is starting, there are even some dancers forming outside" while perfective describes a completed or close to completion activity, e.g. ``The old part has been \textbf{removed} and now there many loose wires now". Table \ref{tab:aspect} shows that progressive aspect is more common in both, but very frequent in DII captions, which aligns with our expectations. 
\begin{table}[!htb]
      \centering
        \begin{tabular}{|r|c|c|}\hline
            Part of Speech   & DII & SIS \\ \hline
            noun   & \textbf{3.85} & 2.73 \\
            preposition  & \textbf{1.75} & 1.01 \\
            adjective   & \textbf{0.98} & 0.85 \\
            personal pronoun   & 0.18 & \textbf{0.80} \\\hline
            \textbf{verb}   &1.55 & \textbf{2.00}\\\hline
            verb base   & 0.07 & \textbf{0.37}\\
            verb gerund  & \textbf{0.61} & 0.23\\
            past tense  & 0.08 & \textbf{0.89}\\
            past participle  &  \textbf{0.21} & 0.17\\
            non-3rd person sing pres  &\textbf{ 0.22}& 0.16\\
            3rd person sing pres  & \textbf{0.36}& 0.19\\
            \hline
        \end{tabular}
    \caption{The difference in part of speech between descriptive and narrative captions. }
    \label{tab:pos_dii_sis}
\end{table}

\begin{table}
  \centering
    %\caption{Using a random sample of 10,000 captions, we observe verb tense and grammatical aspect. The SIS corpora consists of a slightly imbalanced mix of verbs in the past tense form and present tense form, whereas DII is mainly written in the present form. In terms of aspect, both DII and SIS favor progressive aspect where verbs describe ongoing events rather than completed events.}
    \label{tab:verb_tense_distribution}
    \begin{tabular}{|r|c|r|c|c|}\hline
         & past & present  & progressive & perfective \\ \hline
        DII & 18.5\% & \textbf{81.4\%} &  \textbf{94.5\%} & 5.4\%\\
        SIS & \textbf{52.8\%} & 47.2\% &  \textbf{75.1\%} & 24.9\%\\
        \hline
    \end{tabular}
    \caption{Distribution over tense and aspect. }
    \label{tab:aspect}
\end{table}


% \noindent\textbf{Part of Speech (POS).}
% As mentioned in the main text, we extract POS tags over all VIST captions using SpaCy \cite{spacy2} and observe differences in pronoun usage and verb tense between descriptive and narrative captions (Table \ref{tab:pos_dii_sis}). The increased use of pronouns in SIS suggests a deviation from an impersonal, objective tone. Verb tense and aspect also differ between descriptive/narrative captions (Table \ref{tab:verb_tense_distribution}). Past and present tense are both frequent in SIS captions, with more verbs referring to the past than present. Past  and present tense in SIS can occur in the same sentence: ``Afterwards, we take a couple photographs because we paid the photographer to do so." An aligned image would show either show the couple posing for a photo or the transaction. This interaction between past and present occurs over 33\% of SIS captions vs 16\% in DII. 

% Aspect is more evenly distributed in narrative than descriptive captions, but progressive aspect is more common in bother. Progressive aspect refers to verbs that describe an ongoing activity such as ``The event is starting, there are even some dancers forming outside" (SIS) while perfective describes a completed %or close to completion 
% activity, e.g. ``The old part has been \textbf{removed} and now there many loose wires now" (SIS). 

% We hypothesize part of speech tags can be a strong feature to discriminate between DII and SIS, and DII provides more aligned captions since it describes ongoing activities more likely to be present in the accompanying visual scene.

\begin{table}[t]
    \centering
    \scalebox{0.95}{
    \begin{tabular}{|r|c|c|}\hline
        Linguistic features & PREC & REC \\\hline
        POS & \textbf{0.8823} & \textbf{0.8782}\\
        CLIP \cite{Radford2021LearningTV} & 0.7215 & 0.7170 \\\hline
        CLIP+POS & 0.8925 & 0.8893\\
        BERT & \textbf{0.9570} & \textbf{0.9560}
        \\\hline % prec dropped from 0.968 -> 0.957 (previously evaluated on a subset)
    \end{tabular}}
    \caption{We evaluate precision/recall of DII/SIS classifiers on a VIST holdout.}
    %taking in combinations of linguistic features 
    %We see that part of speech tags are quite discriminative, however using all features: RST, CLIP*, and CLUE increase the precision and recall of the classifier. 
    %\cite{Radford2021LearningTV}. 
    \label{tab:dii_sis_classifier}
\end{table}

\input{iccv2023AuthorKit/tables/evaluating_on_pascal_dii_sis}

\subsection{Descriptiveness Classifier}
\textbf{Training details.} We examine using part-of-speech tags to discriminate between descriptive and narrative captions, and compare against methods trained with much more data, BERT \cite{BERT} and CLIP \cite{Radford2021LearningTV}. To set up this task, we use captions from the VIST dataset \cite{huang2016visual} which contains multiple captions written in three distinct styles for each image. We use the descriptive-in-isolation (DII) and story-in-sequence (SIS) captions from VIST \cite{huang2016visual} and assign a positive label (descriptive) to captions drawn from the DII split and a negative label (narrative) to captions drawn from the SIS split. We then train a logistic regression model, which we refer to as the descriptiveness classifier. This classifier takes a binary vector corresponding to the presence of a linguistic feature (e.g. proper noun, adjective, verb - past tense, etc) in the caption. The CLIP-based descriptiveness classifier uses only the cosine similarity between the image embeddings and caption embeddings to distinguish between descriptiveness and narrativeness; training a logistic regression model on a single feature has the effect of finding an appropriate threshold for this task. For the BERT upper bound comparison, we finetune BERT without freezing weights.
For this experiment, we sample a balanced subset of VIST with captions containing an exact match with a category from the following constrained label set: dog, boat, person, car. 
We compare different combinations of the input in Table \ref{tab:dii_sis_classifier}.
We find that simple linguistic features such as part-of-speech do nearly as well as BERT \cite{BERT}, despite being much smaller and having less overhead (no forward pass required). Further, POS is stronger than CLIP, and combining them achieves a better results than either one in combination, indicating these features carry complementary information for this task.

\textbf{WSOD applicability.} For this experiment, we sample a balanced subset of VIST with captions containing an exact match with a category from the following constrained label set: dog, boat, person, car. 
Table \ref{tab:eval_dii_sis_predictions} shows that these classifiers can be used to select quality data for training weakly-supervised object detection models. Each classifier assigns descriptiveness scores; we show that when the highest-scoring caption is selected per image (resulting in a pool of descriptive captions), the results are \textbf{4-6 times better} than when selecting the lowest-scoring captions (resulting in narrative captions). Specifically, we extract labels from the selected captions as pseudo image-level labels using exact string matching, to train the multiple instance detection network using WSDDN \cite{bilen2016weakly}. We measure mAP at $IOU=0.5$ over the selected categories (car, boat, dog, person). 

\textbf{Evaluating the descriptiveness classifier on in-the-wild datasets.}
Seeing the low performance of the descriptiveness classifier in vetting of extracted labels (Table 2 in the main text), we hypothesize that this is due to inability of this classifier to distinguish between descriptive/narrative captions in in-the-wild datasets. We thus test the ability of the part-of-speech based descriptiveness classifier trained on VIST descriptive and narrative captions to predict whether an in-the-wild caption is descriptive. As described in the main text, we label 100 captions as having a descriptive or narrative style from SBUCaps, RedCaps and Conceptual Captions. We use the part-of-speech based classifier trained on VIST to predict whether the annotated captions are descriptive; predictions over the threshold 0.5 are classified as descriptive. We use metrics like accuracy, descriptive misclassification rate ($\frac{\text{\# of incorrect descriptive predictions}}{\text{\# of descriptive captions}}$), and narrative misclassification rate ($\frac{\text{\# of incorrect narrative predictions}}{\text{\# of narrative captions}}$) to evaluate performance.

%We define a narrative style as having subjective elements, first-person perspective ("I", "my", etc), using non-literal expressions ("it's a piece of cake"), assigning intent ("owner shows off her dog"). Note that while VIST-SIS contains examples of narrative-like captions, our definition is inclusive of captions beyond those narrative examples, as real-world captions are not constrained by creating a caption drawing from visible events in previous or future frames. 

% We find that in-the-wild datasets contain far more narrative-like examples than COCO, a heavily descriptive dataset as shown in Table \ref{tab:descriptiveness_in_wild_annot}. RedCaps contains the most narrative-like captions (62\%) in the in-the-wild datasets, whereas ConceptualCaptions contains the least (33\%) we show the ability of our descriptiveness classifier to transfer to these datasets. This is understandable because RedCaps are from a social media source, where people frequently write in a story-like fashion to communicate and connect with others; Conceptual Captions is written with the intent to convey the image, or sometimes the meaning behind the image to visually impaired users using assistive technology. In fact, it's surprising that there's still a considerable amount of narrative-like captions in a heavily preprocessed image-alt text dataset like Conceptual Captions.


\input{iccv2023AuthorKit/tables/descriptiveness_performance.tex} 



 We show the results in Table \ref{tab:desc_classifier_score_in_wild_annot}. We find that while the descriptiveness classifier is able to correctly identify descriptive captions in most datasets, it struggles with correctly identifying narrative captions. We suspect that this might be due to the domain shift from VIST-SIS to the narratives found in the real world. Furthermore, the features that indicate narrativeness in the natural captions are not represented by part-of-speech features. For example, specific words indicate subjectivety, like ``interesting" and others are concrete ``red", yet both are considered adjectives in terms of part-of-speech. Similarly, first-person pronouns like ``I" and ``my" fall under personal pronouns. But, beyond the part of speech tags, there are implicit first-person perspectives found in the grammatically incorrect short hand writing found in natural captions: ``watching a doggie show in the bar while waiting for the pizza". The underspecification of the features used for the descriptiveness classifier explains why it fails to generalize to narrative captions in-the-wild.



==> iccv2023AuthorKit/tables/clip_in_the_wild.tex <==
\begin{table}[]
    \small
    \centering
    \begin{tabular}{c|c|c}\toprule
         \textbf{Dataset} & \textbf{Descriptive} & \textbf{Narrative} \\ \hline
         VIST & 0.303 $\pm$ 0.034 & 0.263 $\pm$ 0.045 \\ \hline
         SBUCaps & 0.306 $\pm$ 0.040 & 0.296 $\pm$ 0.039 \\
         RedCaps & 0.301 $\pm$ 0.039 & 0.286 $\pm$ 0.032 \\
         CC      & 0.300 $\pm$ 0.045 & 0.287 $\pm$ 0.050 \\\bottomrule
    \end{tabular}
    \caption{Visual-text alignment of annotated descriptive and narrative captions from VIST and in-the-wild datasets.}
    \label{tab:clip_in_the_wild}
\end{table}

==> iccv2023AuthorKit/tables/descriptiveness_performance.tex <==
% \begin{table}[]
%     \centering
%     \begin{tabular}{|c|c|c|} \hline
%         Dataset & Narrative (\%) \\\hline
%         COCO & 5 \\\hline
%         CC & 33 \\\hline
%         SBUCaps & 37 \\\hline
%         RedCaps & 62  \\\hline
%     \end{tabular}
%     \caption{From sample of 100 captions, we annotate 100 with descriptive or narrative labels. We find that COCO is dominated by descriptive captions and the in-the-wild datasets are more diverse, containing narrative-like captions.}
%     \label{tab:descriptiveness_in_wild_annot}
% \end{table}

\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|c|}
    \hline
        Metric & DMR & NMR & Accuracy \\ \hline
        COCO & 0.06 & 0.60 & 0.91 \\ \hline
        CC & 0.15 & 0.64 & 0.69 \\ \hline
        SBUCaps & 0.24 & 0.60 & 0.63 \\ \hline
        RedCaps & 0.53 & 0.32 & 0.60 \\ \hline
    \end{tabular}
    \caption{Using the annotated sets, we evaluate the ability of the descriptiveness classifier to generalize to in-the-wild captions. Except for RedCaps, the part-of-speech based descriptiveness classifier is unable generalize outside of the VIST descriptive/narrative domain. We report misclassification rate for the descriptive captions (DMR) and the narrative captions (NMR), defined in the text.}
    \label{tab:desc_classifier_score_in_wild_annot}
\end{table}

==> iccv2023AuthorKit/tables/dii_sis_classifier_table.tex <==
\begin{table}[t]
    \centering
    \scalebox{0.95}{
    \begin{tabular}{|r|c|c|}\hline
        Linguistic features & PREC & REC \\\hline
        POS & \textbf{0.8823} & \textbf{0.8782}\\
        RST & 0.6281 & 0.5170 \\
        CLUE & 0.6813 & 0.6411 \\
        CLIP \cite{Radford2021LearningTV} & 0.7215 & 0.7170
        \\ \hline
        POS+RST & 0.8838 & 0.8787
        \\
        POS+CLUE & 0.8911  & 0.8879 \\
        POS+RST+CLUE & 0.8916 & 0.8884
        \\
CLIP+POS & 0.8925 & 0.8893
        \\
        CLIP+RST & 0.7360 & 0.7312 
        \\
        CLIP+CLUE & 0.7523 & 0.7480
        \\
        CLIP+POS+RST+CLUE &\textbf{ 0.8982} & \textbf{0.8960}\\\hline
        BERT & \textbf{0.9570} & \textbf{0.9560}
        \\\hline % prec dropped from 0.968 -> 0.957 (previously evaluated on a subset)
    \end{tabular}}
    \caption{We evaluate precision/recall of DII/SIS classifiers on a VIST holdout.}
    %taking in combinations of linguistic features 
    %We see that part of speech tags are quite discriminative, however using all features: RST, CLIP*, and CLUE increase the precision and recall of the classifier. 
    %\cite{Radford2021LearningTV}. 
    \label{tab:dii_sis_classifier}
\end{table}

==> iccv2023AuthorKit/tables/dii_sis_clsf.tex <==
\begin{table}[t]
    \centering
    \small
    \scalebox{0.95}{
    \begin{tabular}{r|c|c}\toprule
        Linguistic features & PREC & REC \\\hline
        POS & \textbf{0.8823} & \textbf{0.8782}\\
        RST & 0.6281 & 0.5170 \\
        CLUE & 0.6813 & 0.6411 \\
        CLIP \cite{Radford2021LearningTV} & 0.7215 & 0.7170 \\
        CLIP+POS+RST+CLUE &\textbf{ 0.8982} & \textbf{0.8960}\\\hline
        BERT & \textbf{0.9570} & \textbf{0.9560}
        \\ % prec dropped from 0.968 -> 0.957 (previously evaluated on a subset)
    \end{tabular}}
    \caption{Precision/recall of DII/SIS classifiers on a VIST holdout.}
    \label{tab:dii_sis_classifier}
\end{table}

==> iccv2023AuthorKit/tables/evaluating_on_pascal_dii_sis.tex <==
\begin{table*}[t]
    \centering
    \scalebox{0.9}{
    \begin{tabular}{|c|c|c|c|}    \hline
         & DII (Highest scoring) & Random & SIS (Lowest scoring) \\\hline
        Ground Truth Labels & \textbf{0.0195} & 0.0105 & 0.0050\\\hline
        POS-based Classifier &\textbf{0.0304} & 0.0105 & 0.0047\\\hline
        CLIP-based Classifier & \textbf{0.0173} & 0.0105 & 0.0043 \\\hline
    \end{tabular}}
    \caption{mAP when evaluating on VOC-07. Random is independent of the classifier descriptive-ness scores, hence is trained only once.}
    \label{tab:eval_dii_sis_predictions}
\end{table*}

==> iccv2023AuthorKit/tables/indirect_evaluation.tex <==
\begin{table*}[h]
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
\textbf{Method} &{\textbf{PASCAL VOC 2007 test}} &\textbf{COCO 2014 Val} \\
\hline
Using Ground Truth For Vetting& \underline{39.97} &  \\
No Vetting & 31.22 &  \\
Large Loss Matters \cite{Kim2022LargeLM} & 28.25 &   \\
LocalCLIP-E \cite{Radford2021LearningTV} & 37.12 & \\
VEIL-Redcaps & 37.77 & \\
VEIL-SBUCaps & \textbf{40.49} &  \\
\hline
\end{tabular}
\end{center}
\caption{WSOD Evaluation on PASCAL VOC 2007 and COCO 2014 Val.}
\label{tab:wsod_eval}
\end{table*}


==> iccv2023AuthorKit/tables/pos_vist.tex <==
\begin{table}[t] %[!htb]
      \centering
        \small
        \begin{tabular}{r c c}\hline
            Part of Speech \vline & Descriptive (DII) & Narrative (SIS) \\ \hline
            noun \vline & \textbf{3.85} & 2.73 \\
            preposition \vline& \textbf{1.75} & 1.01 \\
            adjective \vline & \textbf{0.98} & 0.85 \\
            personal pronoun \vline & 0.18 & \textbf{0.80} \\%\hline
            %\textbf{verb} \vline &1.55 & \textbf{2.00}\\\hline
            verb base \vline & 0.07 & \textbf{0.37}\\
            verb gerund \vline& \textbf{0.61} & 0.23\\
            past tense \vline& 0.08 & \textbf{0.89}\\
            %past participle \vline&  \textbf{0.21} & 0.17\\
            %non-3rd person sing pres \vline&\textbf{ 0.22}& 0.16\\
            %3rd person sing pres \vline& \textbf{0.36}& 0.19\\
        \end{tabular}
    \caption{Part of speech differences in descriptive/narrative caps. }
    \label{tab:pos_dii_sis}
\end{table}

==> iccv2023AuthorKit/tables/pretrained_object_detection_prec_rec_on_select_datasets.tex <==
\begin{table}[t]
    \centering
    \scalebox{0.95}{
    \begin{tabular}{|r|c|c|}\hline
        Linguistic features & PREC & REC \\\hline
        POS & \textbf{0.8823} & \textbf{0.8782}\\
        RST & 0.6281 & 0.5170 \\
        CLUE & 0.6813 & 0.6411 \\
        CLIP \cite{Radford2021LearningTV} & 0.7215 & 0.7170
        \\ \hline
        POS+RST & 0.8838 & 0.8787
        \\
        POS+CLUE & 0.8911  & 0.8879 \\
        POS+RST+CLUE & 0.8916 & 0.8884
        \\
CLIP+POS & 0.8925 & 0.8893
        \\
        CLIP+RST & 0.7360 & 0.7312 
        \\
        CLIP+CLUE & 0.7523 & 0.7480
        \\
        CLIP+POS+RST+CLUE &\textbf{ 0.8982} & \textbf{0.8960}\\\hline
        BERT & \textbf{0.9570} & \textbf{0.9560}
        \\\hline % prec dropped from 0.968 -> 0.957 (previously evaluated on a subset)
    \end{tabular}}
    \caption{We evaluate precision/recall of DII/SIS classifiers on a VIST holdout.}
    %taking in combinations of linguistic features 
    %We see that part of speech tags are quite discriminative, however using all features: RST, CLIP*, and CLUE increase the precision and recall of the classifier. 
    %\cite{Radford2021LearningTV}. 
    \label{tab:dii_sis_classifier}
\end{table}

==> iccv2023AuthorKit/tables/structured_noise.tex <==


boat
bus
dog
car
cat
mAP (on pascal voc detection or recognition depending on row)
Am_sbucaps (det)
0.1465
0.5434
0.2109
0.4503
0.2745
0.2910
Am_sbucaps (rec)
0.8475
0.6816
0.9046
0.8955
0.8574
0.6829
llm (det)
 0.1280
0.1173
0.0648
0.1736
0.0842
0.1809
Llm (rec)
0.7024
0.5504
0.9072
0.8742
0.8981
0.6319


